Precise mass determination for the keystone sub-Neptune planet transiting the mid-type M dwarf G 9-40

Context. Despite being a prominent subset of the exoplanet population discovered in the past three decades, the nature and provenance of sub-Neptune-sized planets are still one of the open questions in exoplanet science. Aims. For planets orbiting bright stars, precisely measuring the orbital and planet parameters of the system is the best approach to distinguish between competing theories regarding their formation and evolution. Methods. We obtained 69 new radial velocity observations of the mid-M dwarf G 9-40 with the CARMENES instrument to measure for the first time the mass of its transiting sub-Neptune planet, G 9-40 b, discovered in data from the K2 mission. Results. Combined with new observations from the TESS mission during Sectors 44, 45, and 46, we are able to measure the radius of the planet to an uncertainty of 3.4% (Rb = 1.900 +- 0.065 Re) and determine its mass with a precision of 16% (Mb = 4.00 +- 0.63 Me). The resulting bulk density of the planet is inconsistent with a terrestrial composition and suggests the presence of either a water-rich core or a significant hydrogen-rich envelope. Conclusions. G 9-40 b is referred to as a keystone planet due to its location in period-radius space within the radius valley. Several theories offer explanations for the origin and properties of this population and this planet is a valuable target for testing the dependence of those models on stellar host mass. By virtue of its brightness and small size of the host, it joins L 98-59 d as one of the two best warm (Teq ~ 400 K) sub-Neptunes for atmospheric characterization with JWST, which will probe cloud formation in sub-Neptune-sized planets and break the degeneracies of internal composition models.

==> table-C16_8748-caha3p5_carmenes-vis-0062-srv-rac-complete_output.tex <==
%\begin{table*}
\begin{sidewaystable}
%\begin{footnotesize}
%\begin{scriptsize}
%\begin{ssmall}
\begin{tiny}
\begin{center}
\caption{Radial velocities and spectral activity indicators measured from CARMENES-VIS spectra with \texttt{serval} and \texttt{raccoon}.
\label{table-complete_serval_output}}
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrrrrrrrr}
\hline
\hline
\noalign{\smallskip}
\multicolumn{1}{c}{BJD$_\mathrm{TDB}$} &
\multicolumn{2}{c}{RV} &
\multicolumn{2}{c}{BIS} &
\multicolumn{2}{c}{CCF\_FWHM} &
\multicolumn{2}{c}{CCF\_CTR} &
\multicolumn{2}{c}{CRX} &
\multicolumn{2}{c}{dlW} &
\multicolumn{2}{c}{$\mathrm{H_{\alpha}}$} &
\multicolumn{2}{c}{$\mathrm{NaD_{1}}$} &
\multicolumn{2}{c}{$\mathrm{NaD_{2}}$} &
\multicolumn{2}{c}{$\mathrm{CaIRT_{1}}$} &
\multicolumn{2}{c}{$\mathrm{CaIRT_{2}}$} &
\multicolumn{2}{c}{$\mathrm{CaIRT_{3}}$} &
\multicolumn{1}{c}{SNR} &
\multicolumn{1}{c}{$\mathrm{T_{exp}}$}\\ 
\multicolumn{1}{c}{-2457000} &
\multicolumn{2}{c}{($\mathrm{m\,s^{-1}}$)} &
\multicolumn{2}{c}{($\mathrm{m\,s^{-1}}$)} &
\multicolumn{2}{c}{($\mathrm{km\,s^{-1}}$)} &
\multicolumn{2}{c}{(\%)} &
\multicolumn{2}{c}{($\mathrm{m\,s^{-1}\,Np^{-1}}$)} &
\multicolumn{2}{c}{($\mathrm{m^2\,s^{-2}}$)} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{---} &
\multicolumn{1}{c}{(@737nm)} &
\multicolumn{1}{c}{(s)}\\ 
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{Val.}\\ 
%\noalign{\smallskip}
\hline
%\noalign{\smallskip}
     1453.68494 &           3.934 &           2.855 &          -1.262 &          11.462 &           3.404 &           0.097 &          19.740 &           0.481 &          69.678 &          27.782 &          -0.013 &           3.696 &           0.898 &           0.005 &           0.362 &           0.020 &           0.252 &           0.020 &           0.609 &           0.004 &           0.462 &           0.004 &           0.435 &           0.004 &            37.2 &          1800.0\\
     1453.70640 &           3.565 &           3.069 &         -10.428 &          15.480 &           3.406 &           0.098 &          19.913 &           0.489 &          57.342 &          31.028 &         -27.949 &           5.715 &           0.904 &           0.007 &           0.449 &           0.037 &           0.278 &           0.037 &           0.616 &           0.005 &           0.459 &           0.006 &           0.432 &           0.005 &            28.4 &          1800.0\\
     1455.70680 &           2.484 &           1.960 &          -2.482 &           8.207 &           3.402 &           0.096 &          19.795 &           0.478 &           5.249 &          19.534 &          -4.899 &           1.957 &           0.908 &           0.004 &           0.252 &           0.012 &           0.168 &           0.011 &           0.620 &           0.003 &           0.465 &           0.003 &           0.438 &           0.003 &            50.7 &          1800.6\\
     1455.72952 &           3.860 &           1.669 &          -9.820 &           8.302 &           3.410 &           0.097 &          19.757 &           0.477 &         -17.757 &          16.071 &          -3.921 &           2.707 &           0.912 &           0.004 &           0.216 &           0.011 &           0.182 &           0.011 &           0.615 &           0.003 &           0.462 &           0.003 &           0.439 &           0.003 &            50.2 &          1799.9\\
     1458.66661 &          -0.491 &           1.837 &          -3.324 &           7.473 &           3.405 &           0.096 &          19.869 &           0.477 &           4.126 &          17.180 &         -10.637 &           2.385 &           0.899 &           0.003 &           0.178 &           0.010 &           0.144 &           0.010 &           0.620 &           0.003 &           0.467 &           0.003 &           0.435 &           0.003 &            55.5 &          1800.2\\
     1462.67440 &           6.042 &           1.649 &         -11.165 &           7.027 &           3.425 &           0.096 &          19.665 &           0.469 &          13.442 &          13.563 &           3.018 &           2.238 &           0.904 &           0.003 &           0.209 &           0.008 &           0.169 &           0.009 &           0.615 &           0.003 &           0.454 &           0.003 &           0.427 &           0.002 &            59.3 &          1800.0\\
     1468.64998 &           2.301 &           2.567 &          -6.104 &          10.735 &           3.416 &           0.097 &          19.725 &           0.476 &         -14.309 &          24.064 &          -4.347 &           3.064 &           0.886 &           0.005 &           0.248 &           0.019 &           0.226 &           0.018 &           0.606 &           0.004 &           0.464 &           0.004 &           0.425 &           0.004 &            39.5 &          1802.0\\
     1468.67382 &           4.749 &           2.143 &          -1.174 &           9.442 &           3.412 &           0.095 &          19.920 &           0.475 &          29.988 &          17.744 &         -15.645 &           3.750 &           0.890 &           0.004 &           0.165 &           0.016 &           0.115 &           0.016 &           0.606 &           0.003 &           0.459 &           0.004 &           0.429 &           0.003 &            44.3 &          1800.0\\
     1469.66456 &          -4.790 &           2.083 &         -13.102 &           9.446 &           3.408 &           0.095 &          19.761 &           0.472 &          34.807 &          20.745 &           1.094 &           2.397 &           0.891 &           0.004 &           0.255 &           0.015 &           0.233 &           0.015 &           0.620 &           0.003 &           0.458 &           0.003 &           0.434 &           0.003 &            44.6 &          1799.9\\
     1469.68703 &          -2.067 &           2.050 &         -12.305 &           8.480 &           3.411 &           0.096 &          19.923 &           0.479 &          -1.522 &          20.987 &         -15.542 &           3.672 &           0.881 &           0.004 &           0.202 &           0.013 &           0.146 &           0.013 &           0.614 &           0.003 &           0.462 &           0.003 &           0.438 &           0.003 &            48.9 &          1800.0\\
     1471.73246 &           4.247 &           2.944 &         -25.163 &          13.118 &           3.388 &           0.096 &          20.126 &           0.484 &          -8.525 &          30.811 &         -27.297 &           4.992 &           0.893 &           0.006 &           0.397 &           0.031 &           0.259 &           0.031 &           0.600 &           0.005 &           0.468 &           0.005 &           0.430 &           0.005 &            32.2 &          1799.9\\
     1493.57395 &         -10.080 &           2.933 &          -8.657 &          11.742 &           3.416 &           0.095 &          19.854 &           0.471 &          -6.538 &          31.237 &          -5.357 &           2.938 &           0.898 &           0.005 &           0.397 &           0.022 &           0.251 &           0.021 &           0.613 &           0.004 &           0.466 &           0.004 &           0.428 &           0.004 &            36.3 &          1799.9\\
     1493.59887 &          -8.050 &           2.566 &           7.337 &          10.538 &           3.422 &           0.094 &          20.037 &           0.471 &           0.482 &          26.691 &         -19.292 &           4.036 &           0.892 &           0.005 &           0.301 &           0.020 &           0.205 &           0.019 &           0.613 &           0.004 &           0.455 &           0.004 &           0.436 &           0.004 &            39.8 &          1800.0\\
     1495.56685 &           6.340 &           2.116 &         -10.725 &           8.760 &           3.422 &           0.095 &          19.933 &           0.474 &           4.660 &          20.531 &         -11.125 &           3.026 &           0.892 &           0.004 &           0.240 &           0.014 &           0.162 &           0.014 &           0.613 &           0.003 &           0.460 &           0.003 &           0.438 &           0.003 &            47.5 &          1799.9\\
     1495.59638 &           2.097 &           1.952 &          -9.143 &           8.964 &           3.428 &           0.096 &          19.877 &           0.476 &         -20.237 &          18.711 &         -13.786 &           3.071 &           0.898 &           0.004 &           0.281 &           0.014 &           0.200 &           0.014 &           0.611 &           0.003 &           0.457 &           0.003 &           0.435 &           0.003 &            46.9 &          1800.0\\
     1496.55884 &           2.142 &           1.971 &           1.761 &           8.704 &           3.427 &           0.096 &          19.784 &           0.472 &         -13.410 &          19.751 &          -3.428 &           2.373 &           0.896 &           0.004 &           0.233 &           0.013 &           0.165 &           0.013 &           0.612 &           0.003 &           0.461 &           0.003 &           0.430 &           0.003 &            48.2 &          1800.0\\
     1496.58177 &           4.676 &           1.965 &          -4.574 &           8.820 &           3.429 &           0.096 &          19.876 &           0.474 &         -12.731 &          19.843 &         -11.867 &           2.903 &           0.894 &           0.004 &           0.284 &           0.015 &           0.210 &           0.015 &           0.615 &           0.003 &           0.461 &           0.003 &           0.438 &           0.003 &            47.3 &          1799.9\\
     1497.56210 &          -2.145 &           2.081 &         -15.810 &           8.426 &           3.418 &           0.095 &          19.910 &           0.473 &           2.411 &          20.756 &         -11.467 &           3.041 &           0.900 &           0.004 &           0.174 &           0.013 &           0.141 &           0.014 &           0.613 &           0.003 &           0.456 &           0.003 &           0.436 &           0.003 &            49.3 &          1799.9\\
     1498.60095 &          -2.301 &           2.154 &         -13.043 &           7.602 &           3.419 &           0.096 &          19.725 &           0.472 &          25.277 &          21.081 &           0.421 &           1.727 &           0.894 &           0.003 &           0.259 &           0.011 &           0.188 &           0.010 &           0.609 &           0.003 &           0.461 &           0.003 &           0.434 &           0.003 &            54.9 &          1800.0\\
     1510.54963 &          -4.643 &           1.675 &          -3.885 &           7.771 &           3.422 &           0.095 &          19.681 &           0.468 &         -15.013 &          16.717 &           4.863 &           2.199 &           0.896 &           0.004 &           0.121 &           0.010 &           0.126 &           0.010 &           0.614 &           0.003 &           0.462 &           0.003 &           0.436 &           0.003 &            54.0 &          1799.9\\
     1510.57188 &          -4.519 &           2.183 &          -5.865 &           8.328 &           3.406 &           0.096 &          19.764 &           0.473 &          20.908 &          22.499 &          -2.565 &           2.970 &           0.900 &           0.004 &           0.166 &           0.012 &           0.137 &           0.012 &           0.612 &           0.003 &           0.466 &           0.003 &           0.437 &           0.003 &            50.4 &          1800.0\\
     1524.42078 &          -3.329 &           2.489 &         -16.819 &           9.790 &           3.412 &           0.095 &          19.804 &           0.472 &          27.452 &          23.816 &          -7.132 &           2.430 &           0.891 &           0.004 &           0.082 &           0.016 &           0.109 &           0.016 &           0.604 &           0.003 &           0.458 &           0.004 &           0.437 &           0.003 &            43.1 &          1800.0\\
     1524.44385 &          -3.844 &           2.532 &           5.286 &           8.441 &           3.418 &           0.096 &          19.787 &           0.475 &          17.561 &          24.384 &          -2.292 &           2.464 &           0.887 &           0.004 &           0.094 &           0.012 &           0.097 &           0.012 &           0.606 &           0.003 &           0.457 &           0.003 &           0.433 &           0.003 &            49.5 &          1800.0\\
     1527.58635 &          -2.822 &           2.238 &         -15.832 &           9.011 &           3.418 &           0.097 &          19.821 &           0.478 &          30.120 &          22.789 &          -4.964 &           2.287 &           0.893 &           0.004 &           0.104 &           0.013 &           0.126 &           0.014 &           0.606 &           0.003 &           0.457 &           0.003 &           0.434 &           0.003 &            46.4 &          1800.0\\
     1527.60927 &          -5.754 &           1.636 &         -10.574 &           8.847 &           3.417 &           0.096 &          19.750 &           0.474 &          14.332 &          16.506 &           0.864 &           2.091 &           0.883 &           0.004 &           0.105 &           0.013 &           0.103 &           0.013 &           0.606 &           0.003 &           0.453 &           0.003 &           0.427 &           0.003 &            47.4 &          1800.0\\
     1528.48608 &          -9.979 &           1.485 &          -8.419 &           7.124 &           3.419 &           0.095 &          19.713 &           0.469 &           9.027 &          14.158 &           0.938 &           1.624 &           0.896 &           0.003 &           0.106 &           0.008 &           0.104 &           0.008 &           0.611 &           0.003 &           0.460 &           0.003 &           0.430 &           0.002 &            58.2 &          1800.0\\
     1528.50840 &          -6.686 &           1.836 &         -10.476 &           7.026 &           3.418 &           0.096 &          19.738 &           0.472 &           1.728 &          17.848 &           3.558 &           2.138 &           0.889 &           0.003 &           0.107 &           0.008 &           0.093 &           0.008 &           0.615 &           0.003 &           0.459 &           0.003 &           0.433 &           0.002 &            59.0 &          1800.0\\
     1541.40341 &           2.723 &           3.411 &          -4.260 &          12.354 &           3.428 &           0.097 &          19.734 &           0.474 &          17.556 &          35.773 &          -6.001 &           3.379 &           0.958 &           0.006 &           0.151 &           0.023 &           0.201 &           0.023 &           0.623 &           0.004 &           0.471 &           0.005 &           0.446 &           0.004 &            34.7 &          1800.0\\
     1541.42598 &          -2.652 &           2.548 &          -3.678 &          11.092 &           3.408 &           0.095 &          19.818 &           0.471 &           2.750 &          25.992 &         -10.871 &           2.745 &           0.927 &           0.005 &           0.134 &           0.019 &           0.131 &           0.019 &           0.620 &           0.004 &           0.472 &           0.004 &           0.437 &           0.004 &            38.5 &          1800.4\\
     1542.48875 &           0.497 &           1.985 &           1.013 &          10.246 &           3.425 &           0.096 &          19.723 &           0.471 &           0.176 &          19.490 &          -1.541 &           1.941 &           0.890 &           0.005 &           0.116 &           0.015 &           0.107 &           0.016 &           0.612 &           0.004 &           0.458 &           0.004 &           0.433 &           0.004 &            41.5 &          1800.0\\
     1542.51829 &          -0.511 &           2.309 &          -7.523 &           8.143 &           3.418 &           0.096 &          19.809 &           0.474 &         -13.236 &          23.209 &          -2.717 &           2.122 &           0.885 &           0.004 &           0.083 &           0.011 &           0.097 &           0.012 &           0.612 &           0.003 &           0.457 &           0.003 &           0.432 &           0.003 &            51.2 &          1800.0\\
     1545.51141 &          -6.181 &           2.749 &          12.005 &           9.215 &           3.423 &           0.097 &          19.780 &           0.477 &          32.136 &          28.068 &          -9.727 &           2.988 &           0.874 &           0.004 &           0.107 &           0.013 &           0.126 &           0.014 &           0.610 &           0.003 &           0.467 &           0.003 &           0.435 &           0.003 &            45.9 &          1799.9\\
     1545.53366 &          -6.836 &           2.155 &         -11.380 &           9.504 &           3.405 &           0.096 &          19.860 &           0.476 &           5.250 &          21.492 &          -8.689 &           2.374 &           0.881 &           0.004 &           0.076 &           0.015 &           0.145 &           0.015 &           0.612 &           0.003 &           0.465 &           0.004 &           0.435 &           0.003 &            44.0 &          1800.0\\
     1546.44637 &           2.874 &           1.832 &         -14.310 &           7.226 &           3.432 &           0.096 &          19.687 &           0.470 &         -14.799 &          18.504 &          -3.907 &           2.263 &           0.894 &           0.003 &           0.105 &           0.009 &           0.106 &           0.009 &           0.613 &           0.003 &           0.461 &           0.003 &           0.434 &           0.002 &            58.0 &          1799.9\\
     1546.46921 &          -0.324 &           2.008 &          -8.556 &           7.598 &           3.424 &           0.095 &          19.770 &           0.469 &          -6.655 &          20.932 &          -5.786 &           2.276 &           0.891 &           0.003 &           0.083 &           0.010 &           0.115 &           0.010 &           0.614 &           0.003 &           0.461 &           0.003 &           0.437 &           0.003 &            54.6 &          1799.9\\
     1553.45292 &           3.326 &           1.998 &          -7.656 &           8.941 &           3.418 &           0.095 &          19.818 &           0.469 &          -7.130 &          20.218 &          -7.257 &           2.427 &           0.873 &           0.004 &           0.088 &           0.013 &           0.109 &           0.013 &           0.615 &           0.003 &           0.459 &           0.003 &           0.433 &           0.003 &            47.0 &          1800.0\\
     1553.47930 &           1.644 &           2.231 &          -6.603 &           8.706 &           3.418 &           0.095 &          19.786 &           0.467 &         -23.826 &          22.529 &          -6.552 &           2.739 &           0.878 &           0.004 &           0.097 &           0.012 &           0.106 &           0.012 &           0.616 &           0.003 &           0.464 &           0.003 &           0.432 &           0.003 &            48.5 &          1800.0\\
     1554.43673 &           3.499 &           1.965 &          -1.681 &           8.717 &           3.436 &           0.096 &          19.702 &           0.469 &         -11.389 &          18.913 &          -5.435 &           2.324 &           0.890 &           0.004 &           0.109 &           0.012 &           0.095 &           0.013 &           0.616 &           0.003 &           0.462 &           0.003 &           0.430 &           0.003 &            48.4 &          1799.9\\
     1554.45899 &           2.932 &           2.053 &          -5.111 &           8.420 &           3.410 &           0.095 &          19.827 &           0.471 &         -19.910 &          20.244 &          -0.860 &           2.590 &           0.882 &           0.004 &           0.092 &           0.012 &           0.097 &           0.012 &           0.617 &           0.003 &           0.460 &           0.003 &           0.434 &           0.003 &            49.5 &          1800.0\\
     1555.42633 &          -1.363 &           2.268 &         -19.839 &           8.336 &           3.408 &           0.095 &          19.765 &           0.471 &         -34.289 &          22.240 &          -9.587 &           2.555 &           0.884 &           0.004 &           0.108 &           0.011 &           0.116 &           0.012 &           0.609 &           0.003 &           0.455 &           0.003 &           0.432 &           0.003 &            50.1 &          1800.0\\
     1555.44973 &          -2.117 &           2.318 &           1.826 &           8.942 &           3.428 &           0.096 &          19.748 &           0.470 &         -11.573 &          23.197 &          -1.949 &           2.083 &           0.884 &           0.004 &           0.117 &           0.013 &           0.100 &           0.013 &           0.616 &           0.003 &           0.463 &           0.003 &           0.430 &           0.003 &            46.7 &          1800.0\\
     1571.43095 &           1.152 &           3.243 &          -7.333 &          15.310 &           3.402 &           0.098 &          19.838 &           0.489 &         -12.931 &          33.665 &          -5.394 &           3.942 &           0.916 &           0.007 &           0.098 &           0.030 &           0.129 &           0.031 &           0.603 &           0.005 &           0.453 &           0.006 &           0.438 &           0.005 &            28.6 &          1799.9\\
     1572.46112 &          -3.621 &           2.205 &          -6.265 &           7.791 &           3.408 &           0.095 &          19.819 &           0.470 &          -4.081 &          21.809 &          -3.106 &           2.481 &           0.912 &           0.004 &           0.088 &           0.010 &           0.109 &           0.011 &           0.617 &           0.003 &           0.455 &           0.003 &           0.437 &           0.003 &            53.3 &          1800.0\\
     1572.48350 &           1.494 &           2.072 &          -4.866 &           9.258 &           3.406 &           0.095 &          19.776 &           0.473 &          -3.231 &          19.942 &          -6.222 &           3.108 &           0.898 &           0.004 &           0.096 &           0.014 &           0.092 &           0.015 &           0.610 &           0.003 &           0.453 &           0.003 &           0.434 &           0.003 &            45.5 &          1799.9\\
     1601.37774 &          -1.545 &           2.143 &          -0.962 &           8.404 &           3.421 &           0.094 &          19.841 &           0.467 &          -5.257 &          21.345 &          -5.489 &           2.123 &           0.870 &           0.004 &           0.115 &           0.012 &           0.128 &           0.012 &           0.601 &           0.003 &           0.464 &           0.003 &           0.431 &           0.003 &            49.8 &          1799.9\\
     1601.40002 &          -2.308 &           2.022 &         -10.244 &           8.113 &           3.421 &           0.095 &          19.793 &           0.468 &          14.596 &          19.841 &          -1.655 &           1.709 &           0.884 &           0.004 &           0.121 &           0.012 &           0.110 &           0.012 &           0.604 &           0.003 &           0.460 &           0.003 &           0.431 &           0.003 &            51.5 &          1799.9\\
     1827.60895 &           6.979 &           2.407 &          -5.749 &           8.624 &           3.445 &           0.095 &          19.676 &           0.463 &         -25.325 &          22.626 &           1.775 &           1.851 &           0.899 &           0.004 &           0.377 &           0.014 &           0.284 &           0.013 &           0.619 &           0.003 &           0.468 &           0.003 &           0.435 &           0.003 &            48.9 &          1800.0\\
     1827.63081 &           6.889 &           1.836 &          -6.143 &           7.999 &           3.438 &           0.095 &          19.711 &           0.465 &         -32.825 &          14.021 &           2.311 &           2.438 &           0.911 &           0.004 &           0.346 &           0.012 &           0.269 &           0.012 &           0.619 &           0.003 &           0.468 &           0.003 &           0.441 &           0.003 &            52.6 &          1799.9\\
     1828.62056 &          12.000 &           2.811 &          -1.472 &          13.215 &           3.431 &           0.095 &          19.499 &           0.459 &          -1.933 &          27.093 &          11.371 &           4.017 &           0.899 &           0.006 &           0.808 &           0.027 &           0.529 &           0.025 &           0.620 &           0.004 &           0.482 &           0.005 &           0.439 &           0.004 &            33.6 &          1800.0\\
     1828.64288 &          13.495 &           2.143 &         -12.437 &           8.630 &           3.425 &           0.095 &          19.722 &           0.466 &         -18.398 &          17.964 &           2.227 &           2.066 &           0.894 &           0.004 &           0.471 &           0.014 &           0.308 &           0.013 &           0.612 &           0.003 &           0.471 &           0.003 &           0.434 &           0.003 &            48.9 &          1800.0\\
     1832.64836 &          -1.695 &           2.344 &         -12.792 &          10.171 &           3.443 &           0.092 &          17.846 &           0.405 &         -26.194 &          21.367 &         146.373 &           9.681 &           0.999 &           0.004 &           0.354 &           0.011 &           0.328 &           0.011 &           0.643 &           0.003 &           0.501 &           0.003 &           0.465 &           0.003 &            46.3 &          1800.0\\
     1832.67223 &           7.014 &           3.580 &           2.522 &          11.558 &           3.450 &           0.090 &          17.235 &           0.383 &         -33.277 &          34.301 &         203.736 &          12.673 &           0.902 &           0.004 &           0.373 &           0.012 &           0.339 &           0.012 &           0.621 &           0.004 &           0.475 &           0.004 &           0.447 &           0.003 &            42.7 &          1800.0\\
     1844.58560 &           8.039 &           4.891 &          10.633 &          17.710 &           3.441 &           0.094 &          19.661 &           0.457 &          -9.657 &          42.971 &          -9.952 &           4.268 &           0.908 &           0.008 &           0.800 &           0.039 &           0.524 &           0.038 &           0.609 &           0.006 &           0.467 &           0.007 &           0.430 &           0.006 &            25.8 &          1800.0\\
     1844.60982 &           8.094 &           4.010 &          -0.344 &          15.149 &           3.422 &           0.095 &          19.661 &           0.468 &          28.181 &          30.200 &         -11.293 &           3.691 &           0.887 &           0.007 &           0.657 &           0.031 &           0.454 &           0.030 &           0.616 &           0.005 &           0.456 &           0.006 &           0.438 &           0.005 &            29.5 &          1800.0\\
     1845.62972 &           4.933 &           2.094 &         -11.276 &           7.303 &           3.428 &           0.095 &          19.851 &           0.469 &          17.611 &          18.500 &         -12.969 &           2.928 &           0.911 &           0.003 &           0.233 &           0.011 &           0.164 &           0.010 &           0.618 &           0.003 &           0.472 &           0.003 &           0.445 &           0.003 &            56.5 &          1799.9\\
     1845.65236 &           6.175 &           2.004 &          -8.235 &           7.891 &           3.430 &           0.095 &          19.781 &           0.468 &          27.083 &          17.036 &          -0.760 &           2.098 &           0.900 &           0.004 &           0.303 &           0.011 &           0.227 &           0.011 &           0.613 &           0.003 &           0.469 &           0.003 &           0.436 &           0.003 &            52.7 &          1800.0\\
     1847.65595 &          -1.586 &           2.057 &           4.082 &           7.815 &           3.421 &           0.096 &          20.098 &           0.480 &          24.496 &          20.146 &         -33.364 &           2.615 &           0.893 &           0.004 &           0.009 &           0.011 &           0.015 &           0.011 &           0.615 &           0.003 &           0.464 &           0.003 &           0.430 &           0.003 &            52.6 &          1800.0\\
     1847.67883 &           2.018 &           2.162 &          -6.840 &           8.339 &           3.428 &           0.096 &          20.089 &           0.480 &         -43.030 &          20.129 &         -33.534 &           2.762 &           0.887 &           0.004 &          -0.047 &          -0.012 &           0.000 &           0.013 &           0.608 &           0.003 &           0.462 &           0.003 &           0.428 &           0.003 &            49.6 &          1800.0\\
     1848.58131 &           2.437 &           1.923 &          -8.688 &           7.864 &           3.425 &           0.094 &          19.806 &           0.465 &          -4.819 &          18.387 &           0.211 &           1.974 &           0.881 &           0.004 &           0.289 &           0.011 &           0.200 &           0.011 &           0.608 &           0.003 &           0.459 &           0.003 &           0.433 &           0.003 &            53.0 &          1800.0\\
     1848.60345 &          -2.489 &           1.791 &          -5.797 &           7.755 &           3.439 &           0.095 &          19.733 &           0.467 &          25.893 &          16.353 &           0.811 &           1.915 &           0.888 &           0.003 &           0.272 &           0.011 &           0.194 &           0.010 &           0.617 &           0.003 &           0.464 &           0.003 &           0.437 &           0.003 &            53.7 &          1800.0\\
     1849.61852 &          -3.601 &           2.249 &          -7.824 &           8.402 &           3.436 &           0.095 &          19.723 &           0.465 &          13.208 &          22.473 &          -2.125 &           2.412 &           0.877 &           0.004 &           0.333 &           0.012 &           0.277 &           0.012 &           0.606 &           0.003 &           0.464 &           0.003 &           0.434 &           0.003 &            50.0 &          1800.0\\
     1849.64087 &          -8.947 &           1.868 &         -13.159 &           7.697 &           3.428 &           0.094 &          19.778 &           0.463 &         -21.078 &          17.379 &          -2.301 &           2.094 &           0.888 &           0.003 &           0.326 &           0.011 &           0.247 &           0.010 &           0.605 &           0.003 &           0.466 &           0.003 &           0.439 &           0.003 &            54.2 &          1800.0\\
%\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
%\end{footnotesize}
%\end{scriptsize}
%\end{ssmall}
\end{tiny}
\end{sidewaystable}
%\end{table*}

